A Synthetic Perspective on $(\infty,1)$-Category Theory: Fibrational and Semantic Aspects

Reasoning about weak higher categorical structures constitutes a challenging task, even to the experts. One principal reason is that the language of set theory is not invariant under the weaker notions of equivalence at play, such as homotopy equivalence. From this point of view, it is natural to ask for a different foundational setting which more natively supports these notions. Our work takes up on suggestions in the original article arXiv:1705.07442 by Riehl--Shulman to further develop synthetic $(\infty,1)$-category theory in simplicial homotopy type theory, including in particular the study of cocartesian fibrations. Together with a collection of analytic results, notably due to Riehl--Verity and Rasekh, it follows that our type-theoretic account constitutes a synthetic theory of fibrations of internal $(\infty,1)$-categories, w.r.t. to an arbitrary Grothendieck--Rezk--Lurie-$(\infty,1)$-topos via Shulman's major result arXiv:1904.07004 about strictification of univalent universes.

==> lex-rezk.tex <==
\section{Co-/cone and co-/slice types}

\begin{definition}[Co-/cone types]
	Let $X$ be a type or a shape and $A$ a type. In a setting such as the present one, a map $u:X \to A$ is sometimes referred to as an \emph{$X$-shaped diagram in $A$}. The cospans
	% https://q.uiver.app/?q=WzAsNixbMCwwLCJBIl0sWzIsMCwiQV5YIl0sWzQsMCwiXFx1bml0Il0sWzYsMCwiXFx1bml0Il0sWzgsMCwiQV5YIl0sWzEwLDAsIkEiXSxbMCwxLCJcXG1hdGhybXtjc3R9X0EiXSxbMiwxLCJ1IiwyXSxbMyw0LCJ1Il0sWzUsNCwiXFxtYXRocm17Y3N0fV9BIiwyXV0=
	\[\begin{tikzcd}
		A && {A^X} && \unit && \unit && {A^X} && A
		\arrow["{\mathrm{cst}_A}", from=1-1, to=1-3]
		\arrow["u"', from=1-5, to=1-3]
		\arrow["u", from=1-7, to=1-9]
		\arrow["{\mathrm{cst}_A}"', from=1-11, to=1-9]
	\end{tikzcd}\]
	give rise to the type the type $A/u \defeq \comma{u}{\cst_A}$ of \emph{cocones in $A$ under $X$}, and, dually  $u/A \defeq \comma{\cst_A}{u}$ of \emph{cones in $A$ over $X$}, resp., defined as comma objects:
	% https://q.uiver.app/?q=WzAsOCxbMCwwLCJ1L0EiXSxbMCwxLCJcXGNzdF9BIFxcdGltZXMgXFx1bml0Il0sWzIsMSwiXFxiaWcoQV5YXFxiaWcpXntcXERlbHRhXjF9IFxcdGltZXMgXFxiaWcoQV5YXFxiaWcpXntcXERlbHRhXjF9Il0sWzIsMCwiXFxiaWcoQV5YKV57XFxEZWx0YV4xfSJdLFs0LDAsIkEvdSJdLFs0LDEsIlxcdW5pdCBcXHRpbWVzIFxcY3N0X0EiXSxbNiwxLCJcXGJpZyhBXlhcXGJpZylee1xcRGVsdGFeMX0gXFx0aW1lcyBcXGJpZyhBXlhcXGJpZylee1xcRGVsdGFeMX0iXSxbNiwwLCJcXGJpZyhBXlgpXntcXERlbHRhXjF9Il0sWzEsMiwiXFxjc3RfQSBcXHRpbWVzIHUiXSxbMCwzXSxbMywyLCJcXGxhbmdsZSBcXHBhcnRpYWxfMSwgXFxwYXJ0aWFsXzAgXFxyYW5nbGUiXSxbMCwxXSxbMCwyLCIiLDAseyJzdHlsZSI6eyJuYW1lIjoiY29ybmVyIn19XSxbNCw1XSxbNSw2LCJ1IFxcdGltZXMgXFxjc3RfQSJdLFs0LDddLFs3LDYsIlxcbGFuZ2xlIFxccGFydGlhbF8xLCBcXHBhcnRpYWxfMCBcXHJhbmdsZSJdLFs0LDYsIiIsMSx7InN0eWxlIjp7Im5hbWUiOiJjb3JuZXIifX1dXQ==
	\[\begin{tikzcd}
		{u/A} && {\big(A^X)^{\Delta^1}} && {A/u} && {\big(A^X)^{\Delta^1}} \\
		{A \times \unit} && {A^X \times A^X} && {\unit \times A} && {A^X \times A^X}
		\arrow["{\cst_A \times u}", from=2-1, to=2-3]
		\arrow[from=1-1, to=1-3]
		\arrow["{\langle \partial_1, \partial_0 \rangle}", from=1-3, to=2-3]
		\arrow[from=1-1, to=2-1]
		\arrow["\lrcorner"{anchor=center, pos=0.125}, draw=none, from=1-1, to=2-3]
		\arrow[from=1-5, to=2-5]
		\arrow["{u \times \cst_A}", from=2-5, to=2-7]
		\arrow[from=1-5, to=1-7]
		\arrow["{\langle \partial_1, \partial_0 \rangle}", from=1-7, to=2-7]
		\arrow["\lrcorner"{anchor=center, pos=0.125}, draw=none, from=1-5, to=2-7]
	\end{tikzcd}\]
\end{definition}

\begin{example}[Co-/slice types]
	For a fixed point $b:B$, the \emph{co-/slice types} are defined as $b/B$ and $B/b$, resp. Note that $b/B \equiv \comma{b}{B}$, and similarly for the slice types.
\end{example}

\section{Limits and colimits}

\section{Left exact Rezk types}

\begin{defn}[Co-/span shape]
	The \emph{span} and \emph{cospan shape}, resp.~are defined as the shapes
	\[ \shpspan \defeq \{ \pair{t}{s}:\mathbb I^2 \; | \; t \jdeq 0 \lor s \jdeq 0 \}, \quad \shpcspan \defeq \{ \pair{t}{s}:\mathbb I^2 \; | \; t \jdeq 1 \lor s \jdeq 1 \}.\]
\end{defn}
Of course there are weak equivalences
\[ \shpspan \equiv \Lambda_0^2, \quad \shpcspan \equiv \Lambda_2^2,\]
but these pairs of shapes do not coincide on the strict level of topes.

\begin{definition}[Pullbacks and pushouts in a Rezk type]
	A \emph{span} $\sigma$ in a Rezk type is a diagram $\sigma: B^\shpspan $. Dually, a cospan $\tau$ is a diagram $\tau: B^\shpcspan$. A \emph{pullback over $\sigma$} in $B$ is a terminal element in the cone type $B/\sigma$. Dually, a \emph{pushout over $\tau$} in $B$ is an initial element in the cocone type $\sigma/B$.
\end{definition}
The type of cones can be rewritten as
\[ B/\sigma \equiv \ndexten{\Delta^1 \times \Delta^1}{B}{\shpcspan}{\sigma} .\]
For a span $\sigma:B^\shpspan$ with $\sigma \jdeq c \stackrel{v}{\leftarrow} a \stackrel{u}{\to} b$, a cocone $\vartheta:\sigma/B$ is given by a span $\vartheta \jdeq c \stackrel{g}{\to} d \stackrel{f}{\leftarrow} b$.

One checks that a cocone square $\vartheta \defeq \angled{x,\iota_0,\iota_1}$ is a pushout square if and only if it satisfies the familiar universal property\footnote{It is possible to provide explicitly a completeley strict description replacing the identity types by strict extensions. This could be done elegantly using a join operation on shapes, as is common in simplicial homotopy type theory, but we will not need this here.} internally to the given Rezk type,:
\[
\isPushout_{B,\sigma}(\vartheta) \equiv \prod_{\kappa \defeq (c \stackrel{g}{\to} x \stackrel{f}{\leftarrow} b):\sigma/B} \isContr \Big( \sum_{\gamma:x \to c} \gamma \circ \iota_0 = f \times \gamma \circ \iota_1 = g  \Big)
\]
One can make similar considerations for pullbacks internal to a Rezk type.
